REX: Designing User-centered Repair and Explanations to Address Robot Failures

Robots in real-world environments continuously engage with multiple users and encounter changes that lead to unexpected conflicts in fulfilling user requests. Recent technical advancements (e.g., large-language models (LLMs), program synthesis) offer various methods for automatically generating repair plans that address such conflicts. In this work, we understand how automated repair and explanations can be designed to improve user experience with robot failures through two user studies. In our first, online study ($n=162$), users expressed increased trust, satisfaction, and utility with the robot performing automated repair and explanations. However, we also identified risk factors -- safety, privacy, and complexity -- that require adaptive repair strategies. The second, in-person study ($n=24$) elucidated distinct repair and explanation strategies depending on the level of risk severity and type. Using a design-based approach, we explore automated repair with explanations as a solution for robots to handle conflicts and failures, complemented by adaptive strategies for risk factors. Finally, we discuss the implications of incorporating such strategies into robot designs to achieve seamless operation among changing user needs and environments.

==> figure_compare.tex <==
\begin{figure*}[!h]
  \includegraphics[width=\textwidth]{figures/compare.png}
%   \vspace{-12pt}
  \caption{\textit{Trust and Satisfaction Score Comparison with Scenario 2 ---} }
  \label{fig:compare}
%   \vspace{-6pt}
\end{figure*}


==> figure_findings.tex <==
\begin{figure*}[!t]
  \includegraphics[width=\textwidth]{figures/all_perscenario.png}
%   \vspace{-12pt}
  \caption{\textit{User Trust and Satisfaction Score Per Scenario ---} Data analysis per scenario with significance patterns.}
  \label{fig:collective}
%   \vspace{-6pt}
\end{figure*}


==> figure_implementation.tex <==
\begin{figure*}[!b]
  \includegraphics[width=\textwidth]{figures/flow.png}
  \caption{\textit{Two types of implementation ---} Both the program synthesis and large language model implementation take a user request and output a generated alternate action, or repair, and explanation. The programming synthesis-based implementation (top) uses preset representations of the world, a knowledge graph to resolve underspecified user requests, and a rule bank to identify conflict. It passes the user request through natural language parsing and dependency analysis. When conflict is detected, the program synthesizer selects an alternate action and generates an explanation based on the information in the rule bank. The LLM-based implementation (bottom) uses two LLM agents, one to detect conflicts and plan repair using prompts that capture a representation of the world and a knowledge graph to resolve underspecified user requests and one to evaluate the repair that the first agent generated using the rule bank. Code, representations, and prompts for both implementations are provided in our OSF Repository (\S\ref{sec:system}). }
%   \vspace{-12pt}
  \label{fig:implementation}
%   \vspace{-6pt}
\end{figure*}


==> figure_teasor.tex <==
\begin{figure*}[!h]
  \includegraphics[width=\textwidth]{figures/teaser_final_dis.pdf}
%   \vspace{-12pt}
 \caption{In this work, we explore how robots might handle conflicts with user requests through automated \textit{repair} and \textit{explanation} strategies. \textit{Left:} In the scenario shown above, the user returns from grocery shopping and requests that the groceries be moved to the kitchen counter. \textit{Middle:} The robot later detects that another member of the household specifically requested nothing to be placed on the counter, and takes an alternative action through program repair. \textit{Right:} Not knowing the reason why for the robot's unexpected actions, the user is left confused. In this work, we aim to understand how automated repair and explanations should be designed to improve user experience with robot failures. We present insights into user-centered strategies for robot repair and explanations to address unforeseen conflicts, applicable in real-world contexts and specific types of risks.}
  \label{fig:teasor}
%   \vspace{-6pt}
\end{figure*}

%In this work, we explore how robots might handle conflicts with user requests through automated \textit{repair} and \textit{explanation} strategies. \textit{Left:} In the scenario shown above, the user returns from grocery shopping and requests that the groceries be moved to the kitchen counter. \textit{Middle:} The robot later detects that another member of the household specifically requested nothing to be placed on the counter, and takes an alternative action through program repair. \textit{Right:} Not knowing the reason why for the robot's unexpected actions, the user is left confused. In this work, we aim to understand how automated repair and explanations should be designed to improve user experience with robot failures. We present insights into user-centered strategies for robot repair and explanations to address unforeseen conflicts, applicable in real-world contexts and specific types of risks.
